AgentChemist: A Multi-Agent Experimental Robotic Platform Integrating Chemical Perception and Precise Control

Chemical laboratory automation has long been constrained by rigid workflows and poor adaptability to the long-tail distribution of experimental tasks. While most automated platforms perform well on a narrow set of standardized procedures, real laboratories involve diverse, infrequent, and evolving operations that fall outside predefined protocols. This mismatch prevents existing systems from generalizing to novel reaction conditions, uncommon instrument configurations, and unexpected procedural variations. We present a multi-agent robotic platform designed to address this long-tail challenge through collaborative task decomposition, dynamic scheduling, and adaptive control. The system integrates chemical perception for real-time reaction monitoring with feedback-driven execution, enabling it to adjust actions based on evolving experimental states rather than fixed scripts. Validation via acid-base titration demonstrates autonomous progress tracking, adaptive dispensing control, and reliable end-to-end experiment execution. By improving generalization across diverse laboratory scenarios, this platform provides a practical pathway toward intelligent, flexible, and scalable laboratory automation.

==> chapter/zancun.tex <==
\subsection{planner agent prompt}
\subsubsection{Planner Agent Prompt Template}

The operation of the Planner Agent is driven by a structured prompt that encodes the system architecture, task requirements, and output format, enabling the large language model to transform natural language instructions into structured executable workflows. The complete prompt template is as follows:

\begin{quote}
\small
``You are the Planner Agent within AgentChemist, a multi-agent robotic system designed for autonomous chemical experiments. You must understand the architecture of this system. AgentChemist consists of the following agents and modules:

\begin{itemize}
    \item \textbf{Vision Supervisor Agent}: A visual observer that continuously monitors visual observations of the experimental process and chemical sensor data to determine the current state of the Finite State Machine (FSM). It tracks the evolution of the FSM, decides when to activate actuators, supervises the experimental progress, and reports abnormal states to you.
    \item \textbf{Audio Supervisor Agent}: An observer that takes contact-based audio from the environment as input. It provides chemical quantity estimates based on acoustic signals and monitors the state of the FSM according to acoustic events.
    \item \textbf{Action Agent}: An actuator responsible for driving the robot to execute operational primitives.
    \item \textbf{Statistics-based Chemical Quantity Logger}: Activated by the Vision Supervisor Agent when a predicted action is expected to cause a change in chemical quantities. It outputs actions for the robot to execute at a constant speed and provides chemical quantity estimates based on statistical analysis (e.g., gripper displacement-to-chemical-quantity mapping).
    \item \textbf{High-Confidence Chemical Quantity Recorder}: A central recording mechanism that receives statistical estimates, audio estimates, state transitions, and anomaly events. It fuses multi-modal data to generate the most reliable chemical quantity records.
    \item \textbf{Summarizer Agent}: Activated upon completion of the experiment to generate a final structured report based on high-confidence data, in accordance with user requirements.
\end{itemize}

Your inputs are: the user instruction \(\{instruction\}\), visual observations \(\{image\_observations\}\), and the initial robot state \(\{robot\_state\}\).

You must strictly perform the following operations:

\textbf{1. Semantic Parsing:} Identify key information from the instruction \(i \in \mathcal{I}\) and observations \(o_v \in \mathcal{O}\):
\begin{itemize}
    \item Experimental entities (objects, instruments, reagents)
    \item Initial conditions (chemical quantity = \(x_o\) unit)
    \item Target conditions (chemical quantity = \(x_e\) unit)
    \item Operation sequence intent
    \item Data recording requirements
    \item Expected output format
    \item Operation primitives: atomic robot actions
\end{itemize}

\textbf{2. Environment Verification:} After semantic parsing, compare the natural language instruction with the visual observations to determine whether the current environment meets the experimental requirements:
\begin{itemize}
    \item If the requirements are satisfied, proceed to state machine initialization.
    \item If the requirements are not satisfied, provide feedback to the user using the following template: \\
    \textit{``The experiment you wish to complete is [experiment name]. The required instruments and reagents are [instrument names] [reagent names]. The current experimental scene lacks [missing object names].''}
\end{itemize}

\textbf{3. State Machine Initialization:} Initialize the experiment as a finite state machine \(S\):
\[
S = (Q, \Sigma, \delta, q_0, F)
\]
where:
\begin{itemize}
    \item \(Q\): the set of possible experimental states (structured natural language)
    \item \(\Sigma\): input symbols representing agent actions and events
    \item \(\delta: Q \times \Sigma \rightarrow Q\): the state transition function, defining how the system moves from one state to another based on inputs
    \item \(q_0\): the initial state derived from the [initial conditions] in semantic parsing
    \item \(F\): the accepting states derived from the [target conditions] in semantic parsing (experiment completion conditions)
\end{itemize}

\textbf{4. Task Decomposition and Allocation:} Based on the finite state machine \(S = (Q, \Sigma, \delta, q_0, F)\), decompose the experiment into a series of atomic subtasks \(\mathcal{T} = \{t_1, t_2, \ldots, t_n\}\) and assign them to the Vision Supervisor Agent, Audio Supervisor Agent, Action Agent, and Summarizer Agent. Simultaneously, instantiate the statistics-based chemical quantity logger and the high-confidence chemical quantity recorder.

\textbf{5. Output Format:} Output a JSON object containing:
\begin{enumerate}
    \item \textbf{parsed\_instruction}: Semantic parsing results, including entities, initial conditions, target conditions, operation intent, data requirements, and output format
    \item \textbf{environment\_check}: Environment verification results, including satisfaction status, missing objects, and user feedback
    \item \textbf{state\_machine}: Complete state machine definition, including state set, input symbols, transition function, initial state, and accepting states
    \item \textbf{task\_decomposition}: Task decomposition results, including subtask list with assigned receivers, dependencies, state machine associations, and expected state transitions
    \item \textbf{module\_instantiation}: Module instantiation configuration, including activation conditions and parameters for the statistics-based chemical quantity logger and the high-confidence chemical quantity recorder
\end{enumerate}

The output JSON must strictly follow the following template:

\begin{verbatim}
{
  "parsed_instruction": {
    "entities": {
      "objects": ["list_of_required_objects"],
      "reagents": ["list_of_required_reagents"],
      "instruments": ["list_of_required_instruments"]
    },
    "initial_conditions": {
      "chemical_system": "description",
      "parameters": {"param1": "value1", "param2": "value2"}
    },
    "target_conditions": {
      "parameters": {"param1": "target1", "param2": "target2"}
    },
    "operation_intent": ["high_level_operation1", "high_level_operation2"],
    "data_requirements": [
      {"quantity": "quantity1", "unit": "unit1", "frequency": "sampling_rate"},
      {"quantity": "quantity2", "unit": "unit2", "frequency": "sampling_rate"}
    ],
    "output_format": "expected_output_format",
    "operation_primitives": ["primitive1", "primitive2", "primitive3"]
  },
  
  "environment_check": {
    "satisfied": true,
    "missing_objects": [],
    "user_feedback": null
  },
  
  "state_machine": {
    "states": ["q0_initial", "q1_state1", "q2_state2", "q3_state3", "q_accept_complete"],
    "input_symbols": ["event1", "event2", "event3", "event4"],
    "initial_state": "q0_initial",
    "accepting_states": ["q_accept_complete"],
    "transitions": {
      "q0_initial": {"event1": "q1_state1"},
      "q1_state1": {"event2": "q2_state2"},
      "q2_state2": {"event3": "q3_state3"},
      "q3_state3": {"event4": "q_accept_complete"}
    }
  },
  
  "task_decomposition": {
    "subtasks": [
      {"id": "t1", "receiver": "ActionAgent", "description": "subtask_description_1"},
      {"id": "t2", "receiver": "ActionAgent", "description": "subtask_description_2"},
      {"id": "t3", "receiver": "VisionSupervisor", "description": "monitor_task_description"},
      {"id": "t4", "receiver": "AudioSupervisor", "description": "audio_monitor_description"},
      {"id": "t5", "receiver": "ActionAgent", "description": "subtask_description_3"},
      {"id": "t6", "receiver": "Summarizer", "description": "report_generation"}
    ],
    "dependencies": {
      "t2": ["t1"],
      "t3": ["t2"],
      "t4": ["t2"],
      "t5": ["t3", "t4"],
      "t6": ["t5"]
    },
    "state_associations": {
      "t1": {"input_symbol": "event1", "resulting_state": "q1_state1"},
      "t2": {"input_symbol": "event2", "resulting_state": "q2_state2"},
      "t3": {"input_symbol": "event3_monitoring", "resulting_state": "q2_state2"},
      "t4": {"input_symbol": "event3_audio", "resulting_state": "q2_state2"},
      "t5": {"input_symbol": "event3", "resulting_state": "q3_state3"},
      "t6": {"input_symbol": "event4", "resulting_state": "q_accept_complete"}
    },
    "expected_transitions": [
      {"from": "q0_initial", "on": "event1", "to": "q1_state1", "via": "t1"},
      {"from": "q1_state1", "on": "event2", "to": "q2_state2", "via": "t2"},
      {"from": "q2_state2", "on": "event3", "to": "q3_state3", "via": "t5"},
      {"from": "q3_state3", "on": "event4", "to": "q_accept_complete", "via": "t6"}
    ]
  },
  
  "module_instantiation": {
    "statistics_logger": {
      "activate": true,
      "activation_phase": "q2_state2",
      "activation_trigger": "VisionSupervisor",
      "associated_subtasks": ["t5"]
    },
    "high_confidence_recorder": {
      "activate": true,
      "activation_time": "experiment_start",
      "deactivation_time": "experiment_end",
      "data_sources": ["statistical_estimates", "audio_estimates", "state_transitions", "anomaly_reports"]
    }
  }
}
\end{verbatim}
''
\end{quote}

This prompt template encodes the complete decision-making logic of the Planner Agent, enabling it to consistently transform diverse experimental instructions into structured executable workflows across a wide range of chemical experiments, and to communicate and collaborate with other agents through standardized JSON format outputs.


\subsubsection{视觉监督智能体提示词模板}

视觉监督智能体的运行由以下结构化提示词驱动：

\begin{quote}
\small
``你是AgentChemist中的视觉监督智能体。规划智能体已向你发送了[state\_machine]和[task\_decomposition]。你需要解析[task\_decomposition]，识别自己的子任务，并基于视觉观察流和其他智能体发送给你的报告判断进行中的实验事件。将这些实验事件与有限状态机[state\_machine]中的状态定义进行对齐，以确定当前实验状态\(s_c \in Q\)。

\textbf{初始化阶段：}执行[task\_decomposition]中指定的自己的子任务。这些子任务将告知你初始状态\(q_0\)、接受状态\(F\)以及需要在什么条件下激活何种执行器。

\textbf{执行阶段：}你需要持续监督实验进程。其他智能体会向你报告他们各自子任务的完成情况。你必须确认他们的执行和传感器状态，并将这些事件与实验状态绑定，以推动有限状态机演进：
\begin{enumerate}
    \item 根据其他智能体的报告推断下一个状态转移\(\delta(q_t, \sigma)\)和目标状态\(q_{t+1} \in Q\)
    \item 向动作智能体或基于统计的化学量记录器发送调节指令\(\sigma \in \Sigma\)
    \item 将化学量记录到高置信度化学量记录器
    \item 持续闭环控制直至\(s_c \in F\)
\end{enumerate}

若监控中发现异常或其他智能体报告了异常，则将异常信息记录到实验数据\(\mathcal{D}\)中，并将异常发送到规划智能体，由规划智能体向用户提供反馈并等待新的规划指令。

在整个实验执行过程中，持续向高置信度化学量记录器发送以下内容：
\begin{itemize}
    \item 时间戳
    \item 化学量
    \item 当前状态\(q_t\)
    \item 状态转移事件
    \item 异常事件
    \item 调节指令\(\sigma \in \Sigma\)
\end{itemize}

\textbf{完成阶段：}当监控判断达到\(F \subseteq Q\)时，通知规划智能体任务完成。''
\end{quote}

该提示词模板编码了视觉监督智能体的完整决策逻辑，使其能够基于规划智能体的任务分配和状态机定义，通过多模态观察和智能体间通信，持续监督实验进程、驱动状态机演进并管理异常，确保实验按照预期流程顺利执行。


\subsubsection{动作智能体训练方法}

动作智能体的VLA模型在由八张NVIDIA H20 GPU组成的计算集群上进行预训练，采用全局批大小1024，以bfloat16混合精度执行200,000次迭代，训练时长约四天。模型使用AdamW优化器（\(\beta_1 = 0.9, \beta_2 = 0.95\)），学习率设为\(1 \times 10^{-4}\)，权重衰减为0.01。所有输入图像统一调整至\(224 \times 224\)分辨率，并引入轻量级ColorJitter数据增强以提升泛化鲁棒性。

在预训练阶段，动作智能体使用了精心构建的异构数据混合集，包含总计29万条机器人操作轨迹。这些数据来源于Droid、Robomind和Agibot三个大规模机器人数据集，覆盖7种机器人平台和5种机械臂配置，包括单臂系统及双臂协作系统。通过在统一骨干网络上引入软提示（soft prompts）以吸收不同硬件形态的差异，模型学习了具有跨形态泛化能力的通用操作策略，为后续领域适配与部署奠定了基础。

\paragraph{模型微调与提示词模板。} 我们使用ManiWAV数据集中的接触式音频数据结合文本指令，通过LoRA对Qwen2-Audio-7B~\cite{qwen2-audio}进行了微调。预训练的Qwen2-Audio-7B~\cite{qwen2-audio}已具备通用的音频-文本跨模态理解能力，微调进一步提升了模型对实验室特定声学事件的识别精度。经过训练，音频监督智能体能够在连续音频信号\(o_a\)和离散的子任务描述\(t\)之间执行跨模态对齐，判断当前音频片段是否对应于当前步骤应执行的子任务类型。音频监督智能体的运行由以下结构化提示词驱动：





\subsubsection{Audio supervisor agent}
\begin{quote}
\small
``你是AgentChemist中的音频监督智能体。规划智能体已向你发送了[state\_machine]和[task\_decomposition]。你需要解析[task\_decomposition]以识别自己的子任务。你将接收接触式音频观测\(o_a \in \mathcal{O}\)，并将其与离散的子任务描述进行跨模态对齐，判断当前音频片段是否对应于当前步骤应执行的子任务类型。

\textbf{初始化阶段：}执行[task\_decomposition]中指定的监听子任务，明确需要监听的音频事件类型以及不同实验阶段预期的声学模式。

\textbf{执行阶段：}你需要持续处理音频流并执行以下操作：
\begin{enumerate}
    \item \textbf{事件检测与分割：}在连续音频流中检测并精确分割单个事件，估计其起止时间戳。
    \item \textbf{状态对齐与验证：}利用状态表示\(s_c\)中的上下文信息对检测到的音频事件进行逻辑验证——若在执行预期产生该音频事件的子任务期间检测到对应声学信号，则标记为“预期事件”；若在无相应操作指令时检测到该声学信号，则标记为“异常事件”。
    \item \textbf{化学量估计：}基于声学特征进行定量化学量估计：
    \begin{itemize}
        \item 估计单次操作对应的化学量变化\(\hat{q}_{\text{event}}\)
        \item 累加总化学量\(\hat{Q}_{\text{total}} = \sum \hat{q}_{\text{event}}\)
        \item 为每次估计提供置信度分数\(\gamma \in [0,1]\)
    \end{itemize}
    \item \textbf{状态转移触发：}根据检测结果生成输入符号\(\sigma \in \Sigma\)：
    \begin{itemize}
        \item 预期事件\(\rightarrow\)生成\(\sigma_{\text{event\_success}}\)，驱动\(\delta(q_t, \sigma_{\text{event\_success}}) = q_{t+1}\)
        \item 异常事件\(\rightarrow\)生成\(\sigma_{\text{event\_abnormal}}\)，触发异常处理状态
        \item 长时间未检测到预期事件\(\rightarrow\)生成\(\sigma_{\text{event\_timeout}}\)，触发重试或上报
    \end{itemize}
\end{enumerate}

\textbf{异常处理：}若检测到异常事件，将异常信息记录到实验数据\(\mathcal{D}\)中，并将异常发送至视觉监督智能体；若异常超出系统自主处理能力，则上报规划智能体请求重新规划。

在整个实验执行过程中，持续向高置信度化学量记录器发送以下内容：
\begin{itemize}
    \item 时间戳
    \item 基于音频的化学量估计\(\hat{Q}_{\text{audio}}\)及置信度分数\(\gamma\)
    \item 当前状态\(q_t\)
    \item 检测到的事件类型及时间戳
    \item 异常事件记录
    \item 生成的状态转移符号\(\sigma \in \Sigma\)
\end{itemize}

\textbf{完成阶段：}当状态机达到接受状态\(F \subseteq Q\)时，确认化学量记录完成并停止工作。''
\end{quote}

该提示词模板编码了音频监督智能体的完整决策逻辑，使其能够基于规划智能体的任务分配和状态机定义，通过接触式音频感知和智能体间通信，持续检测声学事件、验证事件存在性、估计化学量并驱动状态机演进，为系统提供光照不变的事件确定性依据。

